Hierarchical Learning Framework for UAV Detection and Identification

The ubiquity of unmanned aerial vehicles (UAVs) or drones is posing both security and safety risks to the public as UAVs are now used for cybercrimes. To mitigate these risks, it is important to have a system that can detect or identify the presence of an intruding UAV in a restricted environment. In this work, we propose a radio frequency (RF) based UAV detection and identification system by exploiting signals emanating from both the UAV and its flight controller, respectively. While several RF devices (i.e., Bluetooth and WiFi devices) operate in the same frequency band as UAVs, the proposed framework utilizes a semi-supervised learning approach for the detection of UAV or UAV's control signals in the presence of other wireless signals such as Bluetooth and WiFi. The semi-supervised learning approach uses stacked denoising autoencoder and local outlier factor algorithms. After the detection of UAV or UAV's control signals, the signal is decomposed by using Hilbert-Huang transform and wavelet packet transform to extract features from the time-frequency-energy domain of the signal. The extracted feature sets are used to train a three-level hierarchical classifier for identifying the type of signals (i.e., UAV or UAV control signal), UAV models, and flight mode of UAV. To demonstrate the feasibility of the proposed framework, we carried out an outdoor experiment for data collection using six UAVs, five Bluetooth devices, and two WiFi devices. The acquired data is called Cardinal RF (CardRF) dataset, and it is available for public use to foster UAV detection and identification research.

==> name.tex <==

background of RF fingerprinting and the feature extraction method proposed.

UAV can be remote control or autonomously operated



advantage of using telemetry signal is that autonomous UAV emits telemetry signals 



% It should be noted that four out of the five UAS are from the same manufacturer (i.e., DJI). The selection of the UAVs is based on two premises which are:
% \begin{itemize}
%     \item Inter-UAV uniqueness (i.e., UAVs from different manufacturers) simplifies the problem of identifying UAVs from different manufacturers, but makes it difficult to identify UAVs of the same manufacturer or model.
%     \item DJI has the largest market share among UAV manufacturers.
% \end{itemize}

% \begin{table*}
% \setlength{\tabcolsep}{1pt}
% \centering

% \caption{Related work on RF based UAV Detection and Identification.}

% \label{Table_ralated_work}

% % \begin{tabular}{p{2cm}| m{2cm}|m{2cm}|m{2cm}|m{2cm}|m{2cm}}
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \hline
%  Literature & Feature extraction method & \multicolumn{2}{c|}{Type of UAV signals}  & Algorithms & Accuracy & Interference & SNR variation & Inference time \\
%  & & Control & Telemetry &  & & &  &\\
 
%  \hline
%  \cite{medaiyese2021wavelet} &  WST & Yes & No &  SqueezeNet (CNN) &98.9\%& Bluetooth, WiFi  & Yes & Yes\\
%  \hline
% \cite{zhao2018classification}& PCA & N/A & N/A  & AC-WGANs & 95\%& WiFi, unknown signal & Yes & No\\
%  \hline
% \cite{basak2021drone}& spectrogram & N/A & N/A  &  Deep residual neural network & 99\%& WiFi& Yes & No\\

% \hline
% \cite{nemer2021rf}&  & N/A & N/A  & Ensemble learning & 99.2\%& No & No & Yes\\

% \hline
% \cite{soltani2020rf}&  & N/A & N/A  & Multiple NN & 91\%& No & No & Yes\\

% \hline
% \cite{swinney2021unmanned}& PSD and CNN & N/A & N/A  & Logistic regression & 91\%& No & No & Yes\\

% \hline
% \cite{zhou2018unmanned}& CSI& N/A & N/A &  Rule-based algorithm & 86.6\%& WiFi & No &\\


% \hline
 
% \cite{ezuma2019detection}& DWT, statistical features & Yes & No & ML algorithms &98.13\%& Bluetooth, WiFi& Yes&\\
%  \hline
 
 
% \cite{al2019rf}& DFT & N/A & N/A  & DL & 84.5\%&None& No&\\


% \hline
% \cite{allahham2020deep}& DFT and CNN & N/A & N/A  & DL & 94.6\%& None & No& \\

% \hline
% \cite{ozturk2020rf}& spectrogram & Yes & N/A  & CNN & 99.5\%& Bluetooth, WiFi & No& \\
% \hline
% In this work & AE and HHT & Yes & Yes &  LOF and XGBoost &-\%& Bluetooth, WiFi & Yes&\\
% \hline
% \end{tabular}}
%  \vspace{-2mm}
% \end{table*}


% The structure of an AE is like that of a multi-layer perceptron (MLP). However, the number of neurons at the input must be equal to that of the output.
% Determining the number of layer or number of neurons for the latent representation is done through an empirical approach.


% The size of the latent representation must be too large because it might reduce the effectiveness of the AE to extract the most important attributes in the data. Conversely, the latent representation must not be too small in comparison to the input size because the AE might not be able to learn enough attributes that we help the reconstruction of data, hereby leading to a lower quality AE. 


% Constraining an AE is important to extract and detect meaning underlying patterns in data, thereby avoiding the AE from  memorizing the data[14]
% Deep AE also known as stacked AE is stacking one or more AE together or in another way adding more hidden layers to AE. 

% We adopted a shallow training of AE instead of training a single stacked AE at a time which is faster and reduces the risk of overfitting.





% \begin{table}[t!]
% \centering
% \caption{Statistical Features From Wavelet Packet Decomposition.}
% \label{Table_2_wpt_features}
% \begin{tabular}{|p{2.5cm}| m{3cm}|m{2cm}|m{2cm}|}
% \hline
% Features & Formula & Measures\\
% \hline
% Standard deviation($\sigma_{T}$)~& $\left[\frac{1}{N-1}\sum_{i=1}^N (x_{i}-\bar{x})^2\right]^{\frac{1}{2}}$ & Dispersion \\
% Variance & $\frac{1}{N}\sum_{i=1}^N (x_{i}-\mu)^2$ & Dispersion \\
% Peak to peak ($x_{\rm{ppv}}$) & $\rm{max(x_{i})}-\rm{min(x_{i}})$ & Waveform amplitude\\
% Shannon~entropy ($H_s$) & $-\sum_{i=1}^N {x_{i}}^2 \log {x_{i}}^2$ & Uncertainty \\
% \hline
% \end{tabular}
% % \vspace{-3mm}
% \end{table}



% \subsection{Feature Selection Using Minimum Redundancy Maximum Relevance (MRMR) Algorithm }

% Using two or more features are that correlated for ML modeling can lead to redundancy of feature and invariably increase the ML model inference cost \cite{ding2005minimum}. To increase the efficiency to producing a generalized model removing redundant feature is imperative. For this reason, MRMR algorithm is adopted.

% MRMR uses the principle of mutual information to find the optimal subset of features that are mutually and maximally dissimilar in a feature space. These subset of features are dependent variables, the dependent variables are function and effective determinants of a response variable  (i.e., target)  \cite{ding2005minimum}. As its name implies, it prunes or minimizes redundancy in a feature set while also maximizing the relevance (i.e., importance) in a feature space.

% Mutual information measures the reduction in uncertainty for one variable based on the knowledge of the other variable. Given two random discrete variables $x$ and $y$, the mutual information $I$ between the two variables is expressed based on their joint probability distribution $p(x,y)$ and the marginal probability of individual variables (i.e., $p(x)$ and $p(y)$) \cite{ding2005minimum}.

% \begin {equation} \label{eq:mutual_information}
% I(x,y)= \sum_{i,j} {p(x_i,y_j)} \frac{p(x_i,y_j)}{p(x_i)p(y_j)}.
% \end{equation}
 
%  similar variable have their mutual information to be zero and differential variables have their mutual information to be higher.
 



% seven top ranked features using MRMR are used for modeling the hierarchical classifier

% A smaller feature set can cover a larger feature space  by adopting MRMR.




  
% In a classification problem, there are several metrics for evaluating the performance of a classifier. These include 
% In this work, the performance of models is presented using accuracy. Using accuracy can misrepresent the performance of a classifier especially when the test data is skewed, so a confusion matrix is used besides. Because of space limitation, we presented some of the confusion matrices of our models, and also, where the confusion matrix is not shown, we provided the precision, recall, and F1-score of the model, which give the summary of the confusion matrix of the model for a thorough understanding of the model performance.
